Shallow Electronic State Preparation for Quantum Chemistry with Quantum Monte Carlo Pre-Selection

Quantum computers hold great promise for molecular simulation, but noise remains a fundamental obstacle. We introduce a Quantum Monte Carlo (QMC) pre-screening procedure that constructs compact, physically motivated Givens rotation ans\"atze tailored to realistic quantum hardware. By identifying the most important wavefunction contributions early in a QMC simulation, we build circuits that are shallower that conventional alternatives while preserving number symmetry. Benchmarked on Quantinuum System Model H1, QMC-prescreened circuits outperform more complex ans\"atze under realistic noise conditions. The method offers a practical path toward chemical accuracy on quantum devices, by providing an adjustable trade-off between expressivity and circuit depth to generate shallow circuits suited to current high-noise devices, as well as deeper, more expressive circuits that can be deployed on future lower-noise devices.

==> Misc/packages.tex <==
% ****************************** Custom Margin ************************
% \ifsetCustomMargin
%   \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
%   \setFancyHdr % To apply fancy header after geometry package is loaded
% \fi

\setlength\parindent{0pt}
\raggedbottom



%****************** Custom Packages ********************************

\usepackage{braket}
\usepackage[linesnumbered,lined,boxed,commentsnumbered]{algorithm2e}
 \usepackage[mode=buildnew]{standalone}
\usepackage{enumitem} 
\usepackage{array}
\newcolumntype{P}[1]{c}
\usepackage{caption} \captionsetup[table]{skip=10pt}
\captionsetup[table]{labelfont=bf}
\captionsetup[figure]{labelfont=bf}
\usepackage{float}
\usepackage{amsmath}
\usepackage{tikz}
\usetikzlibrary{quantikz2}

%for figure captions
\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.}
\usepackage{subcaption}

%tables
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

\usepackage[version=3]{mhchem} % use \ce{} command for chemical species

\usepackage{siunitx}

%bibligraphy
% \ifuseCustomBib
%    \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib
% \fi

% changes the default name `Bibliography` -> `References'
% \renewcommand{\bibname}{References}

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% *********************** Configure Draft Mode *************

% Uncomment to disable figures in `draft'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


% ******************************** Todo Notes ***************
%% Uncomment the following lines to have todonotes.

% \ifsetDraft
% 	\usepackage[colorinlistoftodos]{todonotes}
% 	\newcommand{\mynote}[1]{\todo[author=emw70,size=\small,inline,color=green!40]{#1}}
% \else
% 	\newcommand{\mynote}[1]{}
% 	\newcommand{\listoftodos}{}
% \fi

% comments

\newcommand{\maf}[1]{\textcolor{red}{[\textbf{MAF:} #1]}}
\newcommand{\eline}[1]{\textcolor{blue}{[\textbf{Eline:} #1]}}
\newcommand{\ajwt}[1]{\textcolor{green}{[\textbf{Alex:} #1]}}
\newcommand{\lila}[1]{\textcolor{purple}{[\textbf{Lila:} #1]}}

\usepackage[utf8]{inputenc}
\usepackage{bm}
\usepackage{xcolor,soul}
\usepackage{chemformula}
\usepackage{amsthm}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage[colorlinks,linkcolor=blue,anchorcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}

\usepackage{cleveref}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{figure}{Fig.}{Figs.}
\Crefname{tabular}{Tab.}{Tabs.}
\usepackage{comment}


\usepackage{titlesec}
\titleformat{\subsubsection}{\it}{}{0em}{}
\titlespacing\subsubsection{0pt}{10pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}

